PVNet: Pixel-wise Voting Network for 6DoF Pose Estimation

This paper addresses the challenge of 6DoF pose estimation from a single RGB image under severe occlusion or truncation. Many recent works have shown that a two-stage approach, which first detects keypoints and then solves a Perspective-n-Point (PnP) problem for pose estimation, achieves remarkable performance. However, most of these methods only localize a set of sparse keypoints by regressing their image coordinates or heatmaps, which are sensitive to occlusion and truncation. Instead, we introduce a Pixel-wise Voting Network (PVNet) to regress pixel-wise unit vectors pointing to the keypoints and use these vectors to vote for keypoint locations using RANSAC. This creates a flexible representation for localizing occluded or truncated keypoints. Another important feature of this representation is that it provides uncertainties of keypoint locations that can be further leveraged by the PnP solver. Experiments show that the proposed approach outperforms the state of the art on the LINEMOD, Occlusion LINEMOD and YCB-Video datasets by a large margin, while being efficient for real-time pose estimation. We further create a Truncation LINEMOD dataset to validate the robustness of our approach against truncation. The code will be avaliable at https://zju-3dv.github.io/pvnet/.

==> figure/occlusion_more.tex <==
\begin{figure*}
	\centering
	\scalebox{0.4}{
		\begin{tabular}{ccccc}
			\includegraphics[width=0.45\linewidth]{figure/occlusion/ape1.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/ape2.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/ape3.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/ape4.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/cat1.png}
			\\\includegraphics[width=0.45\linewidth]{figure/occlusion/cat2.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/cat3.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/cat4.png}
		  	&\includegraphics[width=0.45\linewidth]{figure/occlusion/driller1.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/driller2.png}
			\\\includegraphics[width=0.45\linewidth]{figure/occlusion/driller3.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/driller4.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/duck1.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/duck2.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/duck3.png}
			\\\includegraphics[width=0.45\linewidth]{figure/occlusion/duck4.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/can1.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/can2.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/can3.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/can4.png}
			\\\includegraphics[width=0.45\linewidth]{figure/occlusion/hole1.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/hole2.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/hole3.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/hole4.png}
			&\includegraphics[width=0.45\linewidth]{figure/occlusion/glue1.png}
		\end{tabular}
	} \vspace{1mm}
    \caption{Results on the Occlusion LINEMOD dataset. Green 3D bounding boxes represent the ground truth poses, and blue 3D bounding boxes represent our predictions. It can be seen that our method is quite robust to severe occlusions and cluttered scenes, which demonstrates that the keypoint localization based on dense predictions can handle well occluded objects.}
	\vspace{-0mm}
	\label{fig:occ_supp_result}
\end{figure*}


==> figure/synthetic.tex <==
\begin{figure}
	\centering
    \scalebox{1.0}{
		\begin{tabular}{cc}
			\includegraphics[width=0.45\linewidth]{figure/synthetic/can_4121.jpg}
			&\includegraphics[width=0.45\linewidth]{figure/synthetic/holepuncher_7791.jpg} \\
			\includegraphics[width=0.45\linewidth]{figure/synthetic/fuse_1299.jpg}
			&\includegraphics[width=0.45\linewidth]{figure/synthetic/fuse_1620.jpg}
		\end{tabular}
	} \vspace{1mm}
    \caption{Exemplar images of synthetic training data. Rendered images are shown in the first row. The second row shows the synthetic images generated by the ``Cut and Paste" strategy \cite{dwibedi2017cut}.}
	\vspace{1mm}
	\label{fig:syn_data}
\end{figure}



==> figure/truncation_more.tex <==
\begin{figure*}
	\centering
	\scalebox{0.4}{
		\begin{tabular}{ccccc}
			\includegraphics[width=0.45\linewidth]{figure/truncation/ape1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/ape2.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/can1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/can2.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/cam1.png}
			\\\includegraphics[width=0.45\linewidth]{figure/truncation/cam2.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/cat1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/cat2.png}
		  	&\includegraphics[width=0.45\linewidth]{figure/truncation/driller1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/driller2.png}
			\\\includegraphics[width=0.45\linewidth]{figure/truncation/duck1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/duck2.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/eggbox1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/eggbox2.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/glue1.png}
			\\\includegraphics[width=0.45\linewidth]{figure/truncation/glue2.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/hole1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/hole2.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/iron1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/iron2.png}
			\\\includegraphics[width=0.45\linewidth]{figure/truncation/lamp1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/lamp2.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/phone1.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/phone2.png}
			&\includegraphics[width=0.45\linewidth]{figure/truncation/bench1.png}
		\end{tabular}
	} \vspace{1mm}
    \caption{Results on the Truncation LINEMOD dataset. Green 3D bounding boxes represent the ground truth poses, and blue 3D bounding boxes represent our predictions. Although the objects are severely truncated, our method robustly infers the poses based on the visible parts, which indicates that the direction-field representation well deals with truncation.}
	\vspace{-0mm}
	\label{fig:trun_supp_result}
\end{figure*}


==> table/ycb_result.tex <==
\begin{table}
\begin{center}
\scalebox{0.6}{
\begin{tabular}{|c|ccc|ccc|}
\hline
&\multicolumn{3}{c|}{2D Projection}&\multicolumn{3}{c|}{ADD(-S) AUC} \\ \hline
& PoseCNN & Oberweger & OURS & PoseCNN & Oberweger & OURS \\
object &\cite{xiang2017posecnn}&\cite{oberweger2018making}& &\cite{xiang2017posecnn}&\cite{oberweger2018making}& \\ \hline
002\_master\_chef\_can & 74.2 & 0.09 & 29.7 & \textbf{55.17} & 49.1 & \textbf{81.6} \\ 
003\_cracker\_box & 0.12 & \textbf{64.7} & 50.35 & 52.9 & \textbf{83.6} & 80.5 \\ 
004\_sugar\_box & 7.11 & \textbf{72.2} & 61.25 & 68.3 & 82.0 & \textbf{84.9} \\ 
005\_tomato\_soup\_can & 5.21 & 39.8 & \textbf{60.69} & 66.1 & \textbf{79.7} & 78.2 \\ 
006\_mustard\_bottle & 6.44 & \textbf{87.7} & 82.35 & 80.8 & \textbf{91.4} & 88.3 \\ 
007\_tuna\_fish\_can & 2.96 & 38.9 & \textbf{45.21} & 70.6 & 49.2 & \textbf{62.2} \\ 
008\_pudding\_box & 5.14 & \textbf{78.0} & 52.80 & 62.2 & \textbf{90.1} & 85.2 \\ 
009\_gelatin\_box & 15.80 & 94.8 & \textbf{94.85} & 74.8 & \textbf{93.6} & 88.7 \\ 
010\_potted\_meat\_can & 23.10 & 41.2 & \textbf{62.92} & 59.5 & \textbf{79.0} & 65.1 \\ 
011\_banana & 0.26 & \textbf{10.3} & 8.18 & 72.1 & \textbf{51.9} & 51.8 \\ 
019\_pitcher\_base & 0.00 & 5.4 & \textbf{79.30} & 53.1 & 69.4 & \textbf{91.2} \\ 
021\_bleach\_cleanser & 1.16 & 23.2 & \textbf{37.51} & 50.2 & \textbf{76.1} & 74.8 \\ 
024\_bowl & 4.43 & 26.1 & \textbf{33.99} & 69.8 & 76.9 & \textbf{89.0} \\ 
025\_mug & 0.78 & 29.2 & \textbf{52.98} & 58.4 & 53.7 & \textbf{81.5} \\ 
035\_power\_drill & 3.31 & 69.5 & \textbf{74.74} & 55.2 & 82.7 & \textbf{83.4} \\ 
036\_wood\_block & 0.00 & \textbf{2.1} & 2.06 & 61.8 & 55.0 & \textbf{71.5} \\ 
037\_scissors & 0.00 & 12.1 & \textbf{56.35} & 35.3 & \textbf{65.9} & 54.8 \\ 
040\_large\_marker & 1.38 & 1.9 & \textbf{6.80} & 58.1 & \textbf{56.4} & 35.8 \\ 
051\_large\_clamp & 0.28 & 24.2 & \textbf{44.94} & 50.1 & \textbf{67.5} & 66.3 \\ 
052\_extra\_large\_clamp & 0.58 & 1.3 & \textbf{7.77} & 46.5 & 53.9 & \textbf{53.9} \\
061\_foam\_brick & 0.00 & \textbf{75.0} & 25.00 & 85.9 & \textbf{89.0} & 80.6 \\ \hline
average & 3.72 & 39.4 & \textbf{47.39} & 61.0 & 72.8 & \textbf{73.4} \\ \hline
\end{tabular}
} % scalebox
\end{center}
\caption{The accuracies of our method and the baseline methods on the \textbf{YCB-Video} dataset in terms of the \textbf{2D projection} and \textbf{ADD(-S) AUC} metrics. We consider 024\_bowl, 036\_wood\_block, 051\_large\_clamp, 052\_extra\_large\_clamp and 061\_foam\_brick as symmetric objects, as suggested by \cite{xiang2017posecnn}.}
\vspace{-4mm}
\label{tab:ycb_auc}
\end{table}

